Graph neural networks for laminar flow prediction around random 2D shapes

In the recent years, the domain of fast flow field prediction has been vastly dominated by pixel-based convolutional neural networks. Yet, the recent advent of graph convolutional neural networks (GCNNs) have attracted a considerable attention in the computational fluid dynamics (CFD) community. In this contribution, we proposed a GCNN structure as a surrogate model for laminar flow prediction around 2D obstacles. Unlike traditional convolution on image pixels, the graph convolution can be directly applied on body-fitted triangular meshes, hence yielding an easy coupling with CFD solvers. The proposed GCNN model is trained over a data set composed of CFD-computed laminar flows around 2,000 random 2D shapes. Accuracy levels are assessed on reconstructed velocity and pressure fields around out-of-training obstacles, and are compared with that of standard U-net architectures, especially in the boundary layer area.

==> architecture <==
\begin{figure}
\centering

\begin{tikzpicture}[scale=0.85, node distance=0.15cm, rotate=90, transform shape] 
\tikzstyle{layer}		=[rectangle, rounded corners, thick, text centered]
\tikzstyle{cct}		=[circle, draw=mypurple1,		fill=mypurple4,		inner sep=0pt, very thick, text width=0.2cm]
\tikzstyle{skp}		=[inner sep=0pt, 			outer sep=0pt]
\tikzstyle{inp}		=[rectangle, thick, text centered, inner sep=0pt, 		outer sep=0pt,		text width=2cm, draw=black]
\tikzstyle{outp}		=[rectangle, thick, text centered, inner sep=0pt, 		outer sep=0pt,		text width=2cm, opacity=0.75, draw=black]
\tikzstyle{cv}		=[layer, draw=myblue1,		fill=myblue4, 		text width=2cm]
\tikzstyle{pl}		=[layer, draw=myorange1, 	fill=myorange4,		text width=2cm]
\tikzstyle{connection}	=[thick,draw=mygray1,opacity=0.7,decoration={markings, mark=at position 0.7 with {\arrow{stealth}}},postaction={decorate}]
\tikzstyle{rconnection}=[thick,draw=mygray1,opacity=0.7,decoration={markings, mark=at position 0.25 with {\arrow[xscale=-1]{stealth}}},postaction={decorate}]
\scriptsize
\tikzstyle{space_small}=[yshift=-0.5cm]
\tikzstyle{space_med}=[yshift=-1cm]
\tikzstyle{space_large}=[yshift=-1.5cm]

% Input
\node[inp] 						(inp1)  at (0,0)	{\includegraphics[width=\textwidth]{fig/shape_11017_objet.png}};
\node[inp, yshift=-0.8cm, xshift=0cm] 		(inp2)  		{\includegraphics[width=\textwidth]{fig/shape_11017_x.png}};
\node[inp, yshift=-1.1cm, xshift=0.5cm] 		(inp3)  		{\includegraphics[width=\textwidth]{fig/shape_11017_y.png}};
% Encoder branch
\node[cv, below=of inp3, space_small] 		(c11) 		{Graph Conv, $(4,8)$};
\node[skp] at ($(inp3)!0.5!(c11)$) 		(sk)			{};
\node[pl,  below=of c11]			(p1) 		{Avg Smoothing};

\node[cv, below=of p1, space_small] 		(c21) 	 	{Graph Conv, $(8,16)$};
\node[cct]	at ($(p1)!0.5!(c21)$)		(cct1)		{$+$};
\node[pl,  below=of c21]			(p2) 		{Avg Smoothing};

\node[cv, below=of p2, space_small] 		(c31) 	 	{Graph Conv, $(16,32)$};
\node[cct]	at ($(p2)!0.5!(c31)$)		(cct2)		{$+$};
\node[pl, below=of c31] 			(p3) 		{Avg Smoothing};

\node[cv, below=of p3, space_small] 		(c41) 	 	{Graph Conv, $(32,64)$};
\node[cct]	at ($(p3)!0.5!(c41)$)		(cct3)		{$+$};
\node[pl, below=of c41] 			(p4) 		{Avg Smoothing};

% Flow decoder branch
\node[cv, below=of p4, space_small] 		(c52) 	 	{Graph Conv, $(64,64)$};
\node[cct]	at ($(p4)!0.5!(c52)$)		(cct4)		{$+$};
\node[pl, below=of c52] 			(p5) 		{Avg Smoothing};

\node[cv, below=of p5,space_small]	 	(c62) 	 	{Graph Conv, $(64,32)$};
\node[cct]	at ($(p5)!0.5!(c62)$)		(cct5)		{$+$};
\node[pl, below=of c62] 			(p6) 	 	{Avg Smoothing};

\node[cv, below=of p6,space_small]	 	(c72) 	 	{Graph Conv, $(32,16)$};
\node[cct]	at ($(p6)!0.5!(c72)$)		(cct6)		{$+$};
\node[pl, below=of c72] 			(p7) 	 	{Avg Smoothing};

\node[cv, below=of p7,space_small]	 	(c82) 	 	{Graph Conv, $(16,8)$};
\node[cct]	at ($(p7)!0.5!(c82)$)		(cct7)		{$+$};
\node[pl, below=of c82] 			(p8) 	 	{Avg Smoothing};

\node[cv, below=of p8, space_small] 		(c91) 	 	{$1\times1$ conv};
\node[cct]	at ($(p8)!0.5!(c91)$)		(cct8)		{$+$};

\node[outp, below=of c91, yshift=-0.5cm, xshift=-0.5cm] 		(outp2)  		{\includegraphics[width=\textwidth]{fig/shape_11017_p.png}};
\node[outp, below=of c91, yshift=-0.8cm, xshift=0cm] 		(outp3)  		{\includegraphics[width=\textwidth]{fig/shape_11017_v.png}};
\node[outp, below=of c91, yshift=-1.1cm, xshift=0.5cm] 		(outp4)  		{\includegraphic s[width=\textwidth]{fig/shape_11017_u.png}};

% Arrows
\draw[connection]  (inp3.south) -- (c11.north);
\draw[connection]  (p1.south) -- (c21.north);
\draw[connection]  (p2.south) -- (c31.north);
\draw[connection]  (p3.south) -- (c41.north);
\draw[connection]  (p4.south) -- (c52.north);
\draw[connection]  (p5.south) -- (c62.north);
\draw[connection]  (p6.south) -- (c72.north);
\draw[connection]  (p7.south) -- (c82.north);
\draw[connection]  (p8.south) -- (c91.north);

\draw[connection]  (c91.south) to[out=-90,in=90] (outp2.north);
\draw[connection]  (c91.south) to[out=-90,in=90] (outp3.north);
\draw[connection]  (c91.south) to[out=-90,in=90] (outp4.north);

\def\myshift#1{\raisebox{1ex}}
\draw[rconnection,postaction={decorate,decoration={text along path,text align=center,text color=mypurple1,
										text={|\scriptsize\myshift|concatenate}}}] (cct1.east) to[out=0,in=180] (sk.east);
\draw[rconnection,postaction={decorate,decoration={text along path,text align=center,text color=mypurple1,
										text={|\scriptsize\myshift|concatenate}}}] (cct2.east) to[out=0,in=180] (sk.east);
\draw[rconnection,postaction={decorate,decoration={text along path,text align=center,text color=mypurple1,
										text={|\scriptsize\myshift|concatenate}}}] (cct3.east) to[out=0,in=180] (sk.east);
\draw[rconnection,postaction={decorate,decoration={text along path,text align=center,text color=mypurple1,
										text={|\scriptsize\myshift|concatenate}}}] (cct4.east) to[out=0,in=180] (sk.east);
\draw[rconnection,postaction={decorate,decoration={text along path,text align=center,text color=mypurple1,
										text={|\scriptsize\myshift|concatenate}}}] (cct5.east) to[out=0,in=180] (sk.east);
\draw[rconnection,postaction={decorate,decoration={text along path,text align=center,text color=mypurple1,
										text={|\scriptsize\myshift|concatenate}}}] (cct6.east) to[out=0,in=180] (sk.east);
\draw[rconnection,postaction={decorate,decoration={text along path,text align=center,text color=mypurple1,
										text={|\scriptsize\myshift|concatenate}}}] (cct7.east) to[out=0,in=180] (sk.east);
\draw[rconnection,postaction={decorate,decoration={text along path,text align=center,text color=mypurple1,
										text={|\scriptsize\myshift|concatenate}}}] (cct8.east) to[out=0,in=180] (sk.east);
\end{tikzpicture}

\caption{\textbf{Proposed twin-decoder architecture.}}
\label{fig:architecture}
\end{figure}


==> x.tex <==
\def \tikzexternallastkey {CB2E6B8C3C658E3142F1698867FB9CF9}%

